Existence and Properties of Minimum Action Curves for Degenerate Finsler Metrics

I study a class of action functionals on the space of unparameterized oriented rectifiable curves in R^n. The local action is a degenerate type of Finsler metric that may vanish in certain directions, thus allowing for curves with positive Euclidean length but zero action. Given two sets A_1 and A_2, I develop criteria under which there exists a minimum action curve leading from A_1 to A_2. I then study the properties of these minimizers, and I prove the non-existence of minimizers in some situations. Applied to a geometric reformulation of the quasipotential of large deviation theory, my results can prove the existence and properties of maximum likelihood transition curves between two metastable states in a stochastic process with small noise.

==> comments.tex <==
\newpage

\begin{center}
\underline{TO-DO-LIST:}
\begin{itemize}
\item Add proof of property (iii) of Lemma \ref{superprop}, then polish the Part III.
\item Add more references.
\end{itemize}
\end{center}


